Multiplicative-Additive Proof Equivalence is Logspace-complete, via Binary Decision Trees

Given a logic presented in a sequent calculus, a natural question is that of equivalence of proofs: to determine whether two given proofs are equated by any denotational semantics, ie any categorical interpretation of the logic compatible with its cut-elimination procedure. This notion can usually be captured syntactically by a set of rule permutations. Very generally, proofnets can be defined as combinatorial objects which provide canonical representatives of equivalence classes of proofs. In particular, the existence of proof nets for a logic provides a solution to the equivalence problem of this logic. In certain fragments of linear logic, it is possible to give a notion of proofnet with good computational properties, making it a suitable representation of proofs for studying the cut-elimination procedure, among other things. It has recently been proved that there cannot be such a notion of proofnets for the multiplicative (with units) fragment of linear logic, due to the equivalence problem for this logic being Pspace-complete. We investigate the multiplicative-additive (without unit) fragment of linear logic and show it is closely related to binary decision trees: we build a representation of proofs based on binary decision trees, reducing proof equivalence to decision tree equivalence, and give a converse encoding of binary decision trees as proofs. We get as our main result that the complexity of the proof equivalence problem of the studied fragment is Logspace-complete.

==> mallm_rules.tex <==
\begin{center}
	~
	\hfill
	%
	\begin{prooftree}
		\Hypo{\nalpha,\alpha}
	\end{prooftree}
	%
	\hfill
	%
\begin{prooftree}
		\Hypo{\Gamma,A,B}
		\Infer{1}[$\rparr$]{\Gamma,A\parr B}
	\end{prooftree}
	%
	\hfill
	%
	\begin{prooftree}
		\Hypo{\Gamma,A}
		\Hypo{\Delta,B}
		\Infer{2}[$\otimes$]{\Gamma,\Delta,A\otimes B}
	\end{prooftree}
	%
	\begin{prooftree}
		\Hypo{\Gamma}
		\Infer{1}[$\ex ij$]{\Gamma'}
	\end{prooftree}
	%
	\hfill
	%
	\begin{prooftree}
		\Hypo{\Gamma,A}
		\Infer{1}[$\lplus$]{\Gamma,A\plus B}
	\end{prooftree}
	%
	\hfill
	\begin{prooftree}
		\Hypo{\Gamma,B}
		\Infer{1}[$\rplus$]{\Gamma,A\plus B}
	\end{prooftree}
	%
	\hfill
	%
	\begin{prooftree}
		\Hypo{\Gamma,A}
		\Hypo{\Gamma,B}
		\Infer{2}[$\rlabwith{x}$]{\Gamma,A\labwith{x} B}
	\end{prooftree}
	%
	\hfill
	~
\end{center}


